Discretely Nonlinearly Stable Weight-Adjusted Flux Reconstruction High-Order Method for Compressible Flows on Curvilinear Grids

Provable nonlinear stability bounds the discrete approximation and ensures that the discretization does not diverge. For high-order methods, discrete nonlinear stability and entropy stability, have been successfully implemented for discontinuous Galerkin (DG) and residual distribution schemes, where the stability proofs depend on properties of L2-norms. In this paper, nonlinearly stable flux reconstruction (NSFR) schemes are developed for three-dimensional compressible flow in curvilinear coordinates. NSFR is derived by merging the energy stable FR (ESFR) framework with entropy stable DG schemes. NSFR is demonstrated to use larger time-steps than DG due to the ESFR correction functions. NSFR differs from ESFR schemes in the literature since it incorporates the FR correction functions on the volume terms through the use of a modified mass matrix. We also prove that discrete kinetic energy stability cannot be preserved to machine precision for quadrature rules where the surface quadrature is not a subset of the volume quadrature. This paper also presents the NSFR modified mass matrix in a weight-adjusted form. This form reduces the computational cost in curvilinear coordinates through sum-fcatorization and low-storage techniques. The nonlinear stability properties of the scheme are verified on a nonsymmetric curvilinear grid for the inviscid Taylor-Green vortex problem and the correct orders of convergence were obtained for a manufactured solution. Lastly, we perform a computational cost comparison between conservative DG, overintegrated DG, and our proposed entropy conserving NSFR scheme, and find that our proposed entropy conserving NSFR scheme is computationally competitive with the conservative DG scheme.

==> Body/Results/isentropic_vortex.tex <==
\subsection{Isentropic Vortex -- Orders of Accuracy}\label{sec: OOA}

In this subsection we consider the isentropic vortex problem~\cite[Sec. IV]{spiegel2015survey}, using the general three-dimensional formula from Williams and Jameson~\cite[Sec. 5.A]{williams2013nodal} and the same initial condition from Chan and Wilcox~\cite[Sec. 6.3.1]{chan2019discretely} explicitly written in Eq.~(\ref{eq: isen vortex}). 

\begin{equation}
\begin{split}
   & \rho\left(\bm{x},t\right) = \left(1-\frac{\gamma -1}{2}\Pi^2 \right)^{\frac{1}{\gamma -1}},\\
    &\bm{u}\left( \bm{x},t\right) = \bm{u}_0 + \Pi \bm{r},\\
   & \rho E \left(\bm{x},t\right) = \frac{p_0}{\gamma -1}\left(1 - \frac{\gamma -1}{2}\Pi^2 \right)^{\frac{\gamma}{\gamma -1}} + \frac{\rho}{2}|\bm{u} |,\\
   & \Pi = \Pi_\text{max} e^{\frac{1-\bm{r}\bm{r}^T}{2}},\:\:
    \bm{r} = \begin{pmatrix}
        -\left(y-c_2-v_0 t\right) & x - c_1 - u_0 t & 0
    \end{pmatrix},
\end{split}
    \label{eq: isen vortex}
\end{equation}

\noindent where $\bm{u}=(u, v, w)$, $\Pi_\text{max} = 0.4$, $\bm{u}_0=(0,1,0)$, $p_0=1/\gamma$, and $c_1 = c_2 = 5$.
%where we consider the Shu~\cite{shu1998essentially} variant described in~\cite[Table 1]{spiegel2015survey}. 
We use the three-dimensional curvilinear grid on the domain $[0,10]^3$, with $\beta=1/20$ and we advance the vortex until a final time of $t_f=2$s, with $\gamma = 1.4$. For the surface numerical flux, we add Roe dissipation~\cite{roe1981approximate} to the entropy conserving baseline flux. Although the isentropic vortex used is a two-dimensional problem in physical coordinates, due to the non-symmetric mapping, all three reference directions are activated. We integrate on Gauss-Legendre quadrature nodes with an uncollocated Lagrange modal basis. We used the weight-adjusted mass inverse approximation from Eq.~(\ref{eq: weight-adj ESFR mass}).

We compute the L2-error by,

\begin{equation}
    \text{L}2 -\text{error} = \sqrt{\sum_{m=1}^{M}{\int_{\bm{\Omega}_m}{\left(u_m-u\right)^2 d\bm{\Omega}_m}}}
    =\sqrt{\sum_{m=1}^{M}\left(\bm{u}_m^T-\bm{u}_{exact}^T\right)\bm{W}\bm{J}_m\left(\bm{u}_m-\bm{u}_{exact}\right)}.
\end{equation}

The orders of convergence are presented in Figures~\ref{fig: density OOA} and~\ref{fig: pressure OOA}. We found that $DG$ converged at $\mathcal{O}\left(\left(\Delta x\right)^{p+1}\right)$ for both density and pressure, whereas $c_+$ approached $\mathcal{O}\left(\left(\Delta x\right)^{p+1/2}\right)$. For entropy stable schemes, there is no formal proof of convergence and DG convergence results vary from $p+1/2$ to $p+1$. For example, for entropy stable DG, Crean~\textit{et al}.~\cite{crean2018entropy} got $p+1/2$, and Chan~\cite{chan2018discretely} got $p+1$ only for polynomial degrees less than 5. For $c_+$, the loss in half an order matches those for ESFR without the entropy stability framework, and without the weight-adjusted mass matrix inverse on a Cartesian grid from Lambert and Nadarajah~\cite{lambert2023l2}.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/density_OOA_3_isen.png}
    \caption{3D Isentropic Vortex Density OOA}\label{fig: density OOA}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/pressure_OOA_3D_isen.png}
    \caption{3D Isentropic Vortex Density OOA}\label{fig: pressure OOA}
\end{figure}




\iffalse

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
%   2D Results
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table}
\centering{
%\begin{center} 
 \begin{tabular}{|c|c|c|c|c|c|c|}\toprule
Polynomial Order & Scheme &Cells& L2-Error $\rho$ & Rate & L2-Error $p$ & rate \\ \hline 
%%%%%%%%%%%%%%%%%%
%   DG p=3
%%%%%%%%%%%%%%%%%%
$p=3$ & NSFR $c_\text{DG}$ & 4096 & 0.000413433  &- & 0.00032693 & -\\
\cline{3-7}
&  & & 2.65288e-05& & 2.12517e-05& 3.94\\
\cline{3-7}
&  &  & 1.6375e-06& & 1.29412e-06  &4.04 \\
\cline{3-7}
&  &  & 1.01225e-07 & & 7.95358e-08 & \\
%%%%%%%%%%%%%%%%%%
%   cplus p=3
%%%%%%%%%%%%%%%%%%
\cline{2-7} 
& NSFR $c_+$ &   &0.00426272 &- &  0.00418495& -\\
\cline{3-7}
&  & &  0.000429012&  & 0.000409442 &3.35\\
\cline{3-7}
&  &   & 4.27213e-05 & &4.02707e-05  & 3.35\\
\cline{3-7}
&  & &4.0018e-06 &  &3.73606e-06 &  \\\hline
%%%%%%%%%%%%%%%%%%
%   DG p=4
%%%%%%%%%%%%%%%%%%
$p=4$ & NSFR $c_\text{DG}$ &  &4.99867e-05  &- &  4.12327e-05& -\\
\cline{3-7}
&  && 1.6356e-06 & & 1.21029e-06 &5.09 \\
\cline{3-7}
&  &  &5.06258e-08& & 3.70684e-08 &5.03 \\
\cline{3-7}
&  &  &2.74772e-09  & & 2.52906e-09 & \\
%%%%%%%%%%%%%%%%%%
%   cplus p=4
%%%%%%%%%%%%%%%%%%
\cline{2-7} 
& NSFR $c_+$ &   &  0.000388518 &- & 0.000365836 & -\\
\cline{3-7}
&  & &  1.93371e-05 & & 1.81804e-05 &4.33  \\
\cline{3-7}
&  &   &9.6504e-07  & & 8.90335e-07&4.35 \\
\cline{3-7}
&  & & 4.43678e-08&  &4.07453e-08&  \\\hline
%%%%%%%%%%%%%%%%%%
%   DG p=5
%%%%%%%%%%%%%%%%%%
$p=5$ & NSFR $c_\text{DG}$ &  & 6.9891e-06  &- & 4.9499e-06 & -\\
\cline{3-7}
&  && 1.00657e-07 & & 7.85074e-08 &5.98 \\
\cline{3-7}
&  &  &3.44698e-09& & 3.3028e-09 &4.57 \\
\cline{3-7}
&  &  & 1.50644e-09 & &  1.50629e-09& \\
%%%%%%%%%%%%%%%%%%
%   cplus p=5
%%%%%%%%%%%%%%%%%%
\cline{2-7} 
& NSFR $c_+$ &   & 4.59777e-05  &- & 4.19591e-05 & -\\
\cline{3-7}
&  & &1.14158e-06  & &1.04797e-06& 5.32  \\
\cline{3-7}
&  &   &  2.96097e-08& &2.67365e-08 &5.30 \\
\cline{3-7}
&  & & 2.43779e-09&  & 2.41937e-09&  \\
\bottomrule
\end{tabular} 
 %\end{center} 
 }
 \caption{OOA $p=3,4$,$5$ 2D Curvilinear Mesh} \label{tab: OOA}
 \end{table} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%   3D Results
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5


\begin{table}
\centering{
%\begin{center} 
 \begin{tabular}{|c|c|c|c|c|c|c|}\toprule
Polynomial Order & Scheme &Cells& L2-Error $\rho$ & Rate & L2-Error $p$ & rate \\ \hline 
%%%%%%%%%%%%%%%%%%
%   DG p=3
%%%%%%%%%%%%%%%%%%
$p=3$ & NSFR $c_\text{DG}$ & 4096 & 0.00138989 &- & 0.00111843& -\\
\cline{3-7}
&  &32768& 8.93076e-05& & 7.32159e-05&3.93\\
\cline{3-7}
&  &  &5.55114e-06& & 4.51286e-06 &4.02 \\
\cline{3-7}
&  &  &  & &  & \\
%%%%%%%%%%%%%%%%%%
%   cplus p=3
%%%%%%%%%%%%%%%%%%
\cline{2-7} 
& NSFR $c_+$ &   & 0.013347 &- & 0.0131592& -\\
\cline{3-7}
&  & &0.00134026  & &0.00128354 &  3.36\\
\cline{3-7}
&  &   & 0.000131086 & &0.000124116 & 3.37\\
\cline{3-7}
&  & & &  & &  \\\hline
%%%%%%%%%%%%%%%%%%
%   DG p=4
%%%%%%%%%%%%%%%%%%
\cline{3-7}
&  &  &0.00386844& & 0.0035073 & \\
$p=4$ & NSFR $c_\text{DG}$ & 4096 & 0.000165046 &- & 0.000138439&4.66\\
\cline{3-7}
&  &&5.52424e-06 & &4.1437e-06 &5.06\\
\cline{3-7}
&  &  && &  & \\
\cline{3-7}
&  &  &  & &  & \\
%%%%%%%%%%%%%%%%%%
%   cplus p=4
%%%%%%%%%%%%%%%%%%
\cline{3-7}
&  &   & 0.0229301 & &0.0255734 & \\
\cline{2-7} 
& NSFR $c_+$ &   & 0.00124225 &- & 0.00117128& 4.45\\
\cline{3-7}
&  & & 5.99479e-05 & &5.66553e-05 & 4.40 \\
\cline{3-7}
&  &   &  & & & \\
\cline{3-7}
&  & & &  & &  \\\hline
%%%%%%%%%%%%%%%%%%
%   DG p=5
%%%%%%%%%%%%%%%%%%
\cline{3-7}
&  &  &0.00104108& &0.000942044  & \\
$p=5$ & NSFR $c_\text{DG}$ &  & 2.37202e-05 &- &1.68062e-05 & 5.81\\
\cline{3-7}
&  &&3.45441e-07 & &2.67502e-07 &5.97\\
\cline{3-7}
&  &  && &  & \\
\cline{3-7}
&  &  &  & &  & \\
%%%%%%%%%%%%%%%%%%
%   cplus p=5
%%%%%%%%%%%%%%%%%%
\cline{3-7}
&  &  &0.0064271& & 0.00656345 & \\
\cline{2-7} 
& NSFR $c_+$ &   &0.000145652  &- & 0.000134133& 5.61\\
\cline{3-7}
&  & & 3.57985e-06 & &3.31119e-06& 5.34  \\
\cline{3-7}
&  &   &  & & & \\
\cline{3-7}
&  & & &  & &  \\
\bottomrule
\end{tabular} 
 %\end{center} 
 }
 \caption{OOA $p=3,4$,$5$ 3D Curvilinear Mesh} \label{tab: OOA}
 \end{table} 


\iffalse




\begin{table}[t]
\centering{
%\begin{center} 
 \begin{tabular}{|c|c|c|c|c|c|c|}\toprule
Polynomial Order & Scheme &Cells& L2-Error $\rho$ & Rate & L2-Error $p$ & rate \\ \hline 
%%%%%%%%%%%%%%%%%%
%   DG p=4
%%%%%%%%%%%%%%%%%%
$p=4$ & NSFR $c_\text{DG}$ & 100,0.02 & 0.00068429 &- & 0.000597378& -\\
\cline{3-7}
&  & 400,0.01& 1.95788e-05& & 1.64499e-05& 5.18249\\
\cline{3-7}
&  & 1600,0.005 &5.46046e-07 & &4.26506e-07 &5.26937\\
\cline{3-7}
&  & 6400,0.0025 & 1.6418e-08& & 1.25346e-08&5.09\\
%%%%%%%%%%%%%%%%%%
%   cplus p=4
%%%%%%%%%%%%%%%%%%
\cline{2-7} 
& NSFR $c_+$ & 100,0.02  &0.00490165 &- & 0.00618389& -\\
\cline{3-7}
&  & 400,0.01& 0.000220656& & 0.000192037& 5.01\\
\cline{3-7}
&  & 1600,0.005  & 9.84966e-06& & 9.50133e-06& 4.34\\
\cline{3-7}
&  &6400,0.0025&4.09868e-07& 4.59& 3.89201e-07& 4.61\\\hline
%%%%%%%%%%%%%%%%%%
%   DG p=5
%%%%%%%%%%%%%%%%%%
$p=5$ & NSFR $c_\text{DG}$ & 100, 0.0167 & 0.000108841&- & 0.000106912& -\\
\cline{3-7}
&  &400,0.00833& 1.74781e-06& & 1.43204e-06&6.22 \\
\cline{3-7}
&  & 1600, 0.00416667&2.7129e-08 & & 2.1987e-08&6.025\\
\cline{3-7}
&  & d6400,0.00208333 & 7.3544e-10& 5.21 & 6.9157e-10&4.99\\
%%%%%%%%%%%%%%%%%%
%   cplus p=5
%%%%%%%%%%%%%%%%%%
\cline{2-7} 
& NSFR $c_+$ & dx &0.00116161 &- & 0.000729456& -\\
\cline{3-7}
&  & dx& 1.94088e-05& & 1.80379e-05& 5.33772\\
\cline{3-7}
&  & dx & 4.51668e-07& & 4.29043e-07&5.39377\\
\cline{3-7}
&  & dx &1.0508e-08& & 9.8934e-09&5.44\\
\bottomrule
\end{tabular} 
 %\end{center} 
 }
 \caption{Change in Entropy Results $p=4$,$5$ Cartesian Mesh} \label{tab: OOA}
 \end{table} 

\fi


\iffalse
\noindent to check the orders of convergence of the weight-adjusted NSFR scheme. The grid study is performed on both a Cartesian and the heavily warped curvilinear grid in Fig.~\ref{fig: curv grid}. For the volume two-point flux, we use Ranocha's~\cite{ranocha2022preventing} entropy and kinetic energy preserving flux. For the surface numerical flux we use Ranocha's~\cite{ranocha2022preventing} entropy and kinetic energy preserving flux with added Roe dissipation~\cite{roe1981approximate,ismail2009affordable,chandrashekar2013kinetic}.


\underline{Tables with OOA}

As seen from Table\dots the entropy conserving schemes converge at order $p$ whereas the added Roe dissipation allows the schemes to converge at $p+1$.


\begin{enumerate}
    \item Straight Grid
        \begin{itemize}
            \item OOA $c_{DG}$ and $c_+$ entropy conserving with and without upwinding
        \end{itemize}
    \item Curvilinear Grid
    \begin{itemize}
            \item OOA $c_{DG}$ and $c_+$ entropy conserving with and without upwinding, with and without weight-adjusted
        \end{itemize}
\end{enumerate}

\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
%   DG GL Ra with roe diss 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55

\iffalse

p=4

224 refinement           dt           n_cells    L1_error_density        L2_error_density      Linfty_error_density
225          0 2.0916500663358775e-02     256 0.0137096980719888    - 0.0019442504890113    - 0.0030801760771211    -
226          1 1.0458250331679388e-02    1024 0.0003750275568711 5.19 0.0000648320866377 4.91 0.0001474880680078 4.38
227          2 5.2291251658396938e-03    4096 0.0000095370629706 5.30 0.0000017717558221 5.19 0.0000051835587785 4.83
228          3 2.6145625829198469e-03   16384 0.0000002443969067 5.29 0.0000000531558397 5.06 0.0000001667461829 4.96

229 refinement           dt           n_cells    L1_error_pressure       L2_error_pressure     Linfty_error_pressure
230          0 2.0916500663358775e-02     256 0.0121281002627612    - 0.0015159526024230    - 0.0026103568891448    -
231          1 1.0458250331679388e-02    1024 0.0003410414646767 5.15 0.0000474845916323 5.00 0.0000840037792632 4.96
232          2 5.2291251658396938e-03    4096 0.0000087312778029 5.29 0.0000013518118250 5.13 0.0000030829742930 4.77
233          3 2.6145625829198469e-03   16384 0.0000002207403908 5.31 0.0000000392837882 5.10 0.0000000895860716 5.10

p=5

224 refinement           dt           n_cells    L1_error_density        L2_error_density      Linfty_error_density
225          0 1.7430417219465647e-02     256 0.0028348743352843    - 0.0004088918343773    - 0.0006836845720568    -
226          1 8.7152086097328236e-03    1024 0.0000400026799970 6.15 0.0000057918620141 6.14 0.0000096541344432 6.15
227          2 4.3576043048664118e-03    4096 0.0000005565769107 6.17 0.0000001111197639 5.70 0.0000003891270134 4.63
228          3 2.1788021524332059e-03   16384 0.0000000068265083 6.35 0.0000000016544523 6.07 0.0000000075458645 5.69

229 refinement           dt           n_cells    L1_error_pressure       L2_error_pressure     Linfty_error_pressure
230          0 1.7430417219465647e-02     256 0.0026173037291859    - 0.0003518474429166    - 0.0007731787449347    -
231          1 8.7152086097328236e-03    1024 0.0000398293701733 6.04 0.0000056505186247 5.96 0.0000100262221398 6.27
232          2 4.3576043048664118e-03    4096 0.0000005174657744 6.27 0.0000000873577017 6.02 0.0000002992205261 5.07
233          3 2.1788021524332059e-03   16384 0.0000000063294270 6.35 0.0000000012615224 6.11 0.0000000045122606 6.05


p=6

224 refinement           dt           n_cells    L1_error_density        L2_error_density      Linfty_error_density
225          0 1.4940357616684842e-02     256 0.0005534079682575    - 0.0000751539716967    - 0.0000998123033032    -
226          1 7.4701788083424208e-03    1024 0.0000056040709739 6.63 0.0000010811426287 6.12 0.0000028564904921 5.13
227          2 3.7350894041712104e-03    4096 0.0000000327838065 7.42 0.0000000068200433 7.31 0.0000000292733499 6.61
228          3 1.8675447020856052e-03   16384 0.0000000002451430 7.06 0.0000000000546370 6.96 0.0000000002504069 6.87


229 refinement           dt           n_cells    L1_error_pressure       L2_error_pressure     Linfty_error_pressure
230          0 1.4940357616684842e-02     256 0.0005504645345404    - 0.0000765100169952    - 0.0001486729811744    -
231          1 7.4701788083424208e-03    1024 0.0000051047348648 6.75 0.0000008221541572 6.54 0.0000032489730497 5.52
232          2 3.7350894041712104e-03    4096 0.0000000316917907 7.33 0.0000000055941172 7.20 0.0000000169779246 7.58
233          3 1.8675447020856052e-03   16384 0.0000000002286200 7.12 0.0000000000437865 7.00 0.0000000001673824 6.66
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
%%
%   DG curvilinear Results
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse

p=4

224 refinement           dt           n_cells    L1_error_density        L2_error_density      Linfty_error_density
225          0 2.0916500663358775e-02     256 0.0149097141132122    - 0.0020105505804150    - 0.0026124062824873    -
226          1 1.0458250331679388e-02    1024 0.0005063400667669 4.88 0.0000786970336711 4.68 0.0001804216413928 3.86
227          2 5.2291251658396938e-03    4096 0.0000162832779438 4.96 0.0000026932482060 4.87 0.0000131576843579 3.78
228          3 2.6145625829198469e-03   16384 0.0000004682010360 5.12 0.0000000875509752 4.94 0.0000003291080765 5.32
229 refinement           dt           n_cells    L1_error_pressure       L2_error_pressure     Linfty_error_pressure
230          0 2.0916500663358775e-02     256 0.0132865981800955    - 0.0016167969486983    - 0.0023204509098964    -
231          1 1.0458250331679388e-02    1024 0.0004667941661442 4.83 0.0000596608999190 4.76 0.0000971225090334 4.58
232          2 5.2291251658396938e-03    4096 0.0000151530144675 4.95 0.0000021572929495 4.79 0.0000060290656347 4.01
233          3 2.6145625829198469e-03   16384 0.0000004295917211 5.14 0.0000000673055073 5.00 0.0000002145517186 4.81

p=5

224 refinement           dt           n_cells    L1_error_density        L2_error_density      Linfty_error_density
225          0 1.7430417219465647e-02     256 0.0031523551851046    - 0.0004430205540560    - 0.0006023051600238    -
226          1 8.7152086097328236e-03    1024 0.0000540778826966 5.87 0.0000074216898790 5.90 0.0000169708329160 5.15
227          2 4.3576043048664118e-03    4096 0.0000009739307627 5.80 0.0000001797106032 5.37 0.0000006447104346 4.72
228          3 2.1788021524332059e-03   16384 0.0000000131685573 6.21 0.0000000028176989 6.00 0.0000000149764678 5.43
229 refinement           dt           n_cells    L1_error_pressure       L2_error_pressure     Linfty_error_pressure
230          0 1.7430417219465647e-02     256 0.0029383137707805    - 0.0003851469831503    - 0.0006833036868508    -
231          1 8.7152086097328236e-03    1024 0.0000528496347276 5.80 0.0000068916191756 5.80 0.0000133863846919 5.67
232          2 4.3576043048664118e-03    4096 0.0000009140962093 5.85 0.0000001453788101 5.57 0.0000004018140238 5.06
233          3 2.1788021524332059e-03   16384 0.0000000123504799 6.21 0.0000000022092316 6.04 0.0000000106383238 5.24

p=6

224 refinement           dt           n_cells    L1_error_density        L2_error_density      Linfty_error_density
225          0 1.4940357616684842e-02     256 0.0005989568390086    - 0.0000832270488737    - 0.0000952954931885    -
226          1 7.4701788083424208e-03    1024 0.0000081807700277 6.19 0.0000013957465049 5.90 0.0000032971485942 4.85
227          2 3.7350894041712104e-03    4096 0.0000000642606207 6.99 0.0000000125565003 6.80 0.0000000483294647 6.09
228          3 1.8675447020856052e-03   16384 0.0000000004646679 7.11 0.0000000001032740 6.93 0.0000000005716588 6.40
229 refinement           dt           n_cells    L1_error_pressure       L2_error_pressure     Linfty_error_pressure
230          0 1.4940357616684842e-02     256 0.0006007453633523    - 0.0000867682186515    - 0.0001334764052173    -
231          1 7.4701788083424208e-03    1024 0.0000075404421685 6.32 0.0000010834413649 6.32 0.0000034182466510 5.29
232          2 3.7350894041712104e-03    4096 0.0000000611160468 6.95 0.0000000101995463 6.73 0.0000000362824872 6.56
233          3 1.8675447020856052e-03   16384 0.0000000004361152 7.13 0.0000000000829813 6.94 0.0000000004053295 6.48

\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
%%
%   cplus curvilinear Results
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\fi
